MochiSwarm: A testbed for robotic blimps in realistic environments

Testing aerial robots in tasks such as pickup-and-delivery and surveillance significantly benefits from high energy efficiency and scalability of the deployed robotic system. This paper presents MochiSwarm, an open-source testbed of light-weight robotic blimps, ready for multi-robot operation without external localization. We introduce the system design in hardware, software, and perception, which capitalizes on modularity, low cost, and light weight. The hardware allows for rapid modification, which enables the integration of additional sensors to enhance autonomy for different scenarios. The software framework supports different actuation models and communication between the base station and multiple blimps. The detachable perception module allows independent blimps to perform tasks that involve detection and autonomous actuation. We showcase a differential-drive module as an example, of which the autonomy is enabled by visual servoing using the perception module. A case study of pickup-and-delivery tasks with up to 12 blimps highlights the autonomy of the MochiSwarm without external infrastructures.

==> reviews/CommentsToAuthor.tex <==
Comments to author (Associate Editor)
=====================================

The paper introduces MochiSwarm, a low-cost testbed for
autonomous blimp swarms with modular design. While the
hardware implementation shows promise for applications like
search-and-rescue, reviewers raised some valid concerns
regarding insufficient technical justification, unclear
performance metrics, and inadequate documentation. Please
see reviewers' inputs.


----------------------------------------
Comments on Video Attachment:

Reviewers raised some valid concerns regarding placement of
the paper title in the video and lack of clarity in the
objective of missions in the video.
Comments to author (Editor)

================================

The paper is technically sound.


----------------------------------------
Comments on Video Attachment:

ok

==> reviews/Review22317.tex <==
Reviewer 1 of ICRA 2025 submission 4042

Comments to the author
======================

The study introduces a robotic miniature blimp testbed
called MochiSwarm, designed to support swarm operations.
The authors describe the hardware, software, and autonomy
designs of the blimps. These blimps are tested in
search-and-rescue and pickup-and-delivery tasks. The
prototype features a detachable perception module that
enables egocentric autonomy. Overall, the paper is written
clearly and technically; however, some statements would
benefit from additional clarification.

The manuscript states that the designed vehicles are tested
in a realistic and challenging environment. However, it
does not provide information on control or tracking
performance, nor does it address the success of pickup
tasks without the influence of wind disturbances from air
conditioning units (which may be negligible). Therefore,
the claim that the Mochi blimps are tested in an industrial
highbay is not entirely convincing as a "realistic and
challenging" environment.

-Additionally, the manuscript does not address the effect
of rotor gusts from one blimp on another. Is this effect
considered completely negligible? Did the authors adjust
the controller to account for the changing weight of the
blimp when using the detachable camera?

-To detect targets, the authors implement a color-family
detector by collecting and labeling their dataset. However,
the manuscript does not mention the performance of this
color detector (i.e., accuracy) or the sample size of the
dataset. It would be helpful to include this information.

-The motion planning aspect of the blimps is not well
developed. The process of how the pickup occurs such as the
approaching maneuver and trajectory generation after
detection is not specified.

-The equations of motion for the blimps are presented in
the Dynamics and Control section. At the beginning of this
section, it is mentioned that a simple PID controller
manages the actuator, while later it states that a PD
controller controls angular acceleration and yaw. This may
be a simple typo, but it requires clarification.

-In the control section, it is stated that feedback control
elevates the blimp and changes its yaw direction while the
user commands it to move forward. If this is the case, it
should be clarified that the autonomy of the blimps is
limited to these degrees of freedom and that full
autonomous behavior is not available in this setup. If this
is not the intention, the explanation should be made
broader and clearer; otherwise, it may be misleading.

-In the experiment section, what is meant by "minimal human
operator intervention"? Does this refer only to user
commands to move the blimp forward, or does it include
other types of interventions as well?

Comments on the Video Attachment
================================

The process of picking up targets and then autonomously
delivering them to the goals is not well illustrated in the
video. The autonomous pickup process, in particular, is not
convincing in the video.

==> reviews/Review22321.tex <==
Reviewer 3 of ICRA 2025 submission 4042

Comments to the author
======================

General Comments:
The paper presents an interesting approach to designing a
testbed for lighter-than-air vehicles, but the motivation
and contributions need to be more clearly defined and
supported with detailed data and experiments. The
presentation and language should be revised to improve
clarity and coherence, ensuring that the reader fully
understands the value and potential applications of the
proposed testbed.

Major Remarks:
+ An additional section on related work would enhance this
paper by reviewing previous designs aimed at achieving
lightweight and cost-efficient solutions. This section
should compare the advantages and disadvantages of these
designs to clarify how the current approach builds on or
diverges from prior work. This context would help readers
understand the unique contributions and value of the
proposed testbed.
+ The source code link provided in the paper
(https://github.com/LehighBlimpGroup/BlimpSwarm/tree/docume
ntation) is not accessible, resulting in a "website not
found" error.
+ The absence of a README file in the GitHub repository
(https://github.com/LehighBlimpGroup/balltraining) is a
significant limitation, as it leaves users without clear
instructions on how to set up and test the training
process.
+ The paper would greatly benefit from strengthening its
arguments in each paragraph. Every statement made should be
supported by evidence or reasoning, especially in an
academic context. Phrases such as "we did this" need to be
accompanied by clear explanations of why those actions were
taken, how they were implemented, and what outcomes were
expected. Additionally, it would help to address the
significance of these actions in relation to the overall
goals of the paper. This will not only enhance clarity but
also provide a stronger foundation for the claims made.
+ The paper does not provide sufficient evidence or testing
related to the swarm operation for complex tasks. While the
design is presented, it remains unclear whether the
proposed system can effectively perform in real-world swarm
scenarios, particularly when handling complex operations.
To strengthen the paper, the authors should include testing
or simulations that specifically assess the swarm s
performance in multi-agent, collaborative tasks. This would
help to validate whether the design truly supports swarm
behavior and performs as expected under the intended
operational conditions.
+ The paper requires significant revisions in terms of
presentation and language usage. The exact contributions
should be clearly articulated and supported with concrete
data and experiments to strengthen the argument and provide
clarity for the reader.

Minor Remarks:
+ The abstract does not clarify the purpose or motivation
behind the MochiSwarm design, leaving readers uncertain as
to why this testbed environment was developed or what
specific problems it addresses.
+ The introduction should clearly outline the limitations
of prior research, provide motivation for developing this
specific hardware, and present the potential solution
offered. Currently, it lacks a clear rationale for
designing such hardware and does not explain why cost
efficiency and lightweight features are crucial within this
context or why existing designs fall short. Additionally,
the introduction diverges into hardware specifics, which
would be more appropriately detailed in later sections.
This restructuring could better align with the typical flow
and purpose of an introduction.
+ The selection of electronic components lacks clarity
regarding the rationale for choosing specific items.
+ In the experiments, it is important to clearly define
what constitutes "success" in picking up balloons.
+ The statement about improving reliability by enhancing
inter-robot coordination in the future work section is
vague and lacks specifics. It is unclear how the
coordination between robots will be enhanced or what
specific aspects of reliability will be addressed. The
authors should clarify what they mean by "enhancing
coordination"   for example, does this refer to
communication protocols, task allocation strategies, or
synchronization methods?

Methodological and Technical Comments:
+ The reason for using a Bayesian filter, specifically a
log-odds-ratio filter, should be clearly justified in the
paper. It is important to explain why this particular
filtering approach was chosen over others and how it
benefits the system's performance.
+ The paper should focus more on its primary contribution
and maintain a clear narrative around it, rather than
scattering information that may detract from the main
point. For example, if the source code is a significant
contribution, this should be clearly emphasized, but if
it's a supplementary part of the work, the paper should
prioritize explaining the core ideas, methodologies, and
results. The reader should easily understand what the key
contribution is and how it advances the field, without
getting distracted by tangential details. Clarifying the
relative importance of different sections will strengthen
the overall focus of the paper.
+ What is the reason behind the low success rate observed?
For the case with 4 blimps, 14 pick-up attempts were made,
but only 7 successful pick-ups were achieved with 3
balloons. Similarly, for the case with 4 balloons, there
were 15 attempted pick-ups, but only 6 successful pick-ups
with 3 blimps.

Stylistic Form and Presentation:
+ Certain abbreviations, such as IMU and PCB, are not
defined upon their first usage. Defining each abbreviation
when it first appears would improve clarity and help
readers unfamiliar with these terms better understand the
paper.
+ In Figure 5's caption, the word "The" starts with an
uppercase letter in the middle of the sentence without
reason, creating a typographical inconsistency. 
+ Figure 4 would benefit from a more detailed caption that
clearly outlines each component and its purpose, especially
given its complexity. The current caption should be
expanded to describe the key elements and connections in
the figure, guiding the reader through the information
presented and ensuring that all components and their roles
are easy to interpret without needing to refer back to the
main text.
+ If the paper is focusing on the proposal of the testbed
for lighter-than-air vehicles, the authors should emphasize
the benefits of using this testbed, particularly in
relation to its diverse potential applications. Without a
clear discussion on how this testbed can be applied to
various scenarios and the advantages it offers over
existing methods, readers may lack motivation to adopt this
approach in their own work.

Video Remarks:
+ The video should clearly state the problem being
addressed and the motivation behind the work to ensure
viewers understand the significance and context of the
proposed solution. Without this, the audience may struggle
to grasp the relevance of the research.
+ In most parts of the video, the title of the paper is
placed in the middle of the frame, which distracts from the
background. The focus should be on the background content,
with the title placed more subtly to avoid disrupting the
viewer's attention.

Comments on the Video Attachment
================================

Video Remarks:
+ The video should clearly state the problem being
addressed and the motivation behind the work to ensure
viewers understand the significance and context of the
proposed solution. Without this, the audience may struggle
to grasp the relevan

==> reviews/Review22323.tex <==
Reviewer 4 of ICRA 2025 submission 4042

Comments to the author
======================

Your submission of MochiSwarm presents a contribution to
the field of aerial robotics by introducing an affordable
and extensible testbed for swarm operations using
lighter-than-air vehicles. The emphasis on low cost, light
weight, and rapid modifiability addresses important
practical challenges, making MochiSwarm a potentially
useful platform for various applications such as
search-and-rescue and environmental monitoring.

However, to strengthen your paper and elevate it beyond the
borderline category, consider the following areas for
improvement:

-Theoretical Depth: While the hardware and software
implementations are well-detailed, the theoretical
framework underpinning the swarm algorithms and
coordination mechanisms is relatively shallow. Providing a
more rigorous analysis of the algorithms, including
stability, convergence, and scalability properties, would
enhance the scientific merit of your work.

-Comprehensive Experimental Validation: Your experiments
showcase the basic capabilities of MochiSwarm in controlled
environments. To better demonstrate its effectiveness, it
is crucial to include more extensive real-world
deployments. Testing in diverse and unpredictable settings
would provide stronger evidence of the systems robustness
and adaptability.

-Comparative Analysis: The paper would benefit from a
detailed comparison with existing multi-robot aerial
platforms like Crazyswarm and GRASP micro-UAV. Including
quantitative metrics such as energy efficiency, payload
capacity, communication reliability, and fault tolerance
would help highlight the unique advantages and potential
limitations of MochiSwarm relative to established systems.

Advanced Coordination Strategies: The current coordination
mechanism appears to be relatively simple. Exploring more
sophisticated swarm intelligence techniques or
decentralized control algorithms could improve performance
and reduce the likelihood of issues such as collision and
redundant actions among blimps.

Robustness to Environmental Factors: Addressing how
MochiSwarm handles varying environmental conditions, such
as wind gusts, obstacles, and dynamic target movements,
would make the system more applicable to real-world
scenarios. Including experiments that test these factors
would demonstrate the systems resilience and reliability.

Documentation and Open-Source Contribution: Highlighting
the availability of your hardware designs and software code
in open-source repositories is commendable. Ensuring
comprehensive documentation and user-friendly guides will
facilitate adoption and encourage contributions from the
research community, thereby increasing the impact of your
work.


Comments on the Video Attachment
================================

The video summarizes MochiSwarm, highlighting its low-cost,
lightweight design and swarm coordination capabilities.

==> reviews/Review22327.tex <==
Reviewer 6 of ICRA 2025 submission 4042

Comments to the author
======================

The paper presents MochiSwarm, a testbed designed for swarm
coordination of robotic blimps, particularly for use in
challenging environments. This system features an
Arduino-based design emphasizing low cost, modularity, and
ease of modification. The authors detail the hardware and
software, including a detachable perception module for
autonomous object detection and delivery. The paper
includes experiments that validate the scalability and
resilience of the system in realistic scenarios, such as
pickup-and-delivery tasks.

Strengths:

Innovation and Relevance: The concept of a low-cost,
adaptable blimp swarm testbed is novel and offers potential
applications in search-and-rescue, environmental
monitoring, and logistics.

Detailed Design and Implementation: The paper provides
comprehensive insights into the hardware, software, and
communication architecture, allowing for future
reproducibility. Additionally, the use of ESP-NOW for swarm
communication without external infrastructure is a
practical solution for real-world deployment.

Experimental Validation: The inclusion of
pickup-and-delivery experiments showcases the systems
effectiveness in performing complex tasks in unstructured
environments. The results demonstrate the system's
scalability and robustness, which are critical for swarm
robotics applications.

he paper contributes valuable insights to the field of
swarm robotics with a promising system design and practical
experimental results. 

Comments on the Video Attachment
================================

video was clear and well prepared.

==> reviews/iThenticateScanResult.tex <==
ICRA 2025 has access to the CrossCheck database. Read more about the
CrossCheck initiative to prevent scholarly and professional plagiarism
at http://www.crossref.org/crosscheck.html.

Submission 4042 received a cumulative similarity score 26%.

For more information about the scan, log in at
https://ras.papercept.net with your PIN 283996 and password, enter your
ICRA 2025 author workspace, and select the option 'Inspect the reviews
and decision letter' under 'Choose an option...' for submission 4042.

Similarity scores and scan reports are generated by an external
provider (iThenticate) and not by the conference.

The scan reports are stored on the iThenticate servers and not
downloaded to the conference submission system servers. Eventually the
reports are deleted from the iThenticate servers at a time determined
by conference and provider policy, after which they are no longer
available.

Please check the on-line report to understand how the similarity score
was determined and which sections of your paper may need changes.

The score and report are provided to assist you in revising your
manuscript, if necessary.

The conference will not be able to provide you a score or a report for
the revised manuscript.
